A witness for topological order and stable quantum memories in abelian anyonic systems

We propose a novel parameter, the anyonic topological entropy, designed to detect the error correcting phase of a topological memory. Unlike similar quantities such as the topological entropy, the anyonic topological entropy is defined using the states of the anyon occupations. As such, though the parameter deals with phases and phase transitions that are quantum in nature, it can be calculated solely from classical probability distributions. In many cases, these calculations will be tractable using efficient classical algorithms. The parameter therefore provides a new avenue for efficient studies of anyonic systems.

==> JPAv3(published)/changes <==
The paragraph:

It should be noted that a similar study could be performed for the toric code perturbed by magnetic fields. Though the phase transitions for this case have already been studied \cite{vidal}, the use of the anyonic topological would provide an independent verification of these results and may shed new light on the properties of the model. However, this would require a significant increase of the computation cost compared to the one-dimensional case, and so such a study is deferred to future work.

has been added, as has the reference

\bibitem{vidal} J. Vidal, S. Dusuel, and K. P. Schmidt, Phys. Rev. B \textbf{79}, 033109 (2009).


==> changes <==
The paragraph:

It should be noted that a similar study could be performed for the toric code perturbed by magnetic fields. Though the phase transitions for this case have already been studied \cite{vidal}, the use of the anyonic topological would provide an independent verification of these results and may shed new light on the properties of the model. However, this would require a significant increase of the computation cost compared to the one-dimensional case, and so such a study is deferred to future work.

has been added, as has the reference

\bibitem{vidal} J. Vidal, S. Dusuel, and K. P. Schmidt, Phys. Rev. B \textbf{79}, 033109 (2009).

